BenchMint: From Real-World Tasks to Executable Benchmarks

Large language models (LLMs) need evaluations of everyday reasoning and tool use, such as planning itineraries under user constraints and grounding numerical answers in evidence. We introduce BenchMint, an automated benchmark-construction workflow, and Daily-Life, its collection of 100 selected tasks across 11 real-world domains. BenchMint jointly constructs tasks and scoring criteria from the same source documents. Language-model judges assess possible answers against these criteria using tool traces and private evidence. We report 26 model/harness configurations, including GPT, Claude and Gemini families; 17 have complete domain profiles. These are descriptive configuration results, not a controlled model ranking. In one selected travel task, we corrected the reference total from 320 to 380 minutes while keeping both answers unchanged. The incorrect answer's arithmetic verdict switched from pass to fail; the correct answer's switched from fail to pass. With one ballot per cell, this exposes a reference error without establishing repeatability or collection-wide validity. Incomplete construction comparisons establish no general advantage of joint authoring or feedback-guided revision.

==> revision/arxiv_layout.tex <==
% Local arXiv layout support: keep readable floats beside their interpretation.
\RequirePackage{float}
\RequirePackage{longtable}
\renewcommand{\topfraction}{0.88}
\renewcommand{\bottomfraction}{0.80}
\renewcommand{\textfraction}{0.10}
\renewcommand{\floatpagefraction}{0.95}
\setcounter{topnumber}{2}
\setcounter{totalnumber}{3}
\setlength{\textfloatsep}{10pt plus 2pt minus 2pt}
\setlength{\intextsep}{8pt plus 2pt minus 2pt}
\setlength{\floatsep}{12pt plus 2pt minus 2pt}
% Modest paragraph separation lets the main argument reflow around the full
% configuration table without reducing any body or table font size.
% Applied after the title box, which resets the class paragraph defaults.
% No stretch between floats if a genuinely multipage appendix table is needed.
\makeatletter
\setlength{\@fptop}{0pt}
\setlength{\@fpsep}{12pt}
\makeatother


==> revision/draft_notes.tex <==
% Visible working-draft actions. Resolve each action, then remove its use before submission.
% Input this shared source in the preamble; keep the current font and size.
% There is no visibility switch or automatic note removal.
\RequirePackage{xcolor}
\definecolor{tgDraftNoteRed}{HTML}{B00020}
\DeclareRobustCommand{\tgDraftNote}[2]{%
  \begingroup
    \color{tgDraftNoteRed}%
    [#1] #2%
  \endgroup
}


==> revision/numbers.tex <==
% GENERATED FILE — do not edit by hand.
% Source: analysis/claim_ledger.json   Regenerate: make numbers
% Every claim-bearing number in the paper must come from \num{<claim_id>}.

\makeatletter
% \num{claim_id} → ledger 里的值;未登记的 key 渲染成醒目红字,
% 绝不静默展开成空串(那是错数字上线的经典路径)。
\newcommand{\num}[1]{%
  \ifcsname claimval@#1\endcsname
    \csname claimval@#1\endcsname
  \else
    \textcolor{red}{\textbf{[UNKNOWN CLAIM: \detokenize{#1}]}}%
  \fi}

\expandafter\gdef\csname claimval@axis.A_n\endcsname{5{,}966}
\expandafter\gdef\csname claimval@axis.B_n\endcsname{7{,}748}
\expandafter\gdef\csname claimval@axis.C_fail_paired_pct\endcsname{55.7}
\expandafter\gdef\csname claimval@axis.C_fail_pct\endcsname{30.9}
\expandafter\gdef\csname claimval@axis.C_n\endcsname{7{,}483}
\expandafter\gdef\csname claimval@axis.D_n\endcsname{12{,}274}
\expandafter\gdef\csname claimval@axis.E_n\endcsname{4{,}068}
\expandafter\gdef\csname claimval@axis.F_n\endcsname{601}
\expandafter\gdef\csname claimval@axis.G_n\endcsname{8{,}183}
\expandafter\gdef\csname claimval@axis.H_n\endcsname{67}
\expandafter\gdef\csname claimval@axis.I_n\endcsname{1{,}917}
\expandafter\gdef\csname claimval@axis.J_n\endcsname{5{,}650}
\expandafter\gdef\csname claimval@axis.YC_gap_paired_pp\endcsname{20.9}
\expandafter\gdef\csname claimval@axis.YC_gap_pp\endcsname{45.7}
\expandafter\gdef\csname claimval@axis.Y_fail_paired_pct\endcsname{76.6}
\expandafter\gdef\csname claimval@axis.Y_fail_pct\endcsname{76.6}
\expandafter\gdef\csname claimval@axis.Y_n\endcsname{1{,}186}
\expandafter\gdef\csname claimval@axis.n_runs_C\endcsname{3756}
\expandafter\gdef\csname claimval@axis.n_runs_Y\endcsname{687}
\expandafter\gdef\csname claimval@axis.n_runs_matched\endcsname{685}
\expandafter\gdef\csname claimval@cap.n_cells\endcsname{231}
\expandafter\gdef\csname claimval@cap.n_items\endcsname{100}
\expandafter\gdef\csname claimval@cap.n_models\endcsname{21}
\expandafter\gdef\csname claimval@cap.n_pairs\endcsname{210}
\expandafter\gdef\csname claimval@cap.n_subsets\endcsname{11}
\expandafter\gdef\csname claimval@capoff.C_disagree_pct\endcsname{3.87}
\expandafter\gdef\csname claimval@capoff.n_solvers\endcsname{13}
\expandafter\gdef\csname claimval@capoff.n_verdict_solvers\endcsname{6}
\expandafter\gdef\csname claimval@capoff.n_verdicts\endcsname{55{,}104}
\expandafter\gdef\csname claimval@capoff.top_overall\endcsname{68\%}
\expandafter\gdef\csname claimval@capoff.verdict_top_pass_pct\endcsname{74.7}
\expandafter\gdef\csname claimval@cost.judge_max_usd\endcsname{\$69.87}
\expandafter\gdef\csname claimval@cost.judge_mean_usd\endcsname{\$5.25}
\expandafter\gdef\csname claimval@cost.judge_median_usd\endcsname{\$4.39}
\expandafter\gdef\csname claimval@cost.judge_p75_usd\endcsname{\$6.28}
\expandafter\gdef\csname claimval@cost.judge_p95_usd\endcsname{\$10.54}
\expandafter\gdef\csname claimval@cost.n_priced\endcsname{3{,}789}
\expandafter\gdef\csname claimval@cost.total_judge_usd\endcsname{\$19{,}890}
\expandafter\gdef\csname claimval@drift.n_neg\endcsname{7}
\expandafter\gdef\csname claimval@drift.n_pairs\endcsname{16}
\expandafter\gdef\csname claimval@drift.n_pos\endcsname{7}
\expandafter\gdef\csname claimval@drift.sign_p\endcsname{1.00}
\expandafter\gdef\csname claimval@hr.C_ci_hi\endcsname{6.39}
\expandafter\gdef\csname claimval@hr.C_ci_lo\endcsname{2.32}
\expandafter\gdef\csname claimval@hr.C_n\endcsname{362}
\expandafter\gdef\csname claimval@hr.Y_ci_hi\endcsname{4.09}
\expandafter\gdef\csname claimval@hr.Y_ci_lo\endcsname{0.32}
\expandafter\gdef\csname claimval@hr.Y_disagree_pct\endcsname{1.15}
\expandafter\gdef\csname claimval@hr.Y_n\endcsname{174}
\expandafter\gdef\csname claimval@hr.agreement_pct\endcsname{97.5}
\expandafter\gdef\csname claimval@hr.frac_perfect_pct\endcsname{76.4}
\expandafter\gdef\csname claimval@hr.n_decided\endcsname{2,942}
\expandafter\gdef\csname claimval@hr.n_items\endcsname{212}
\expandafter\gdef\csname claimval@hr.n_reviewers\endcsname{6}
\expandafter\gdef\csname claimval@hr.too_loose_n\endcsname{46}
\expandafter\gdef\csname claimval@hr.too_strict_n\endcsname{29}
\expandafter\gdef\csname claimval@infra.api_error\endcsname{69}
\expandafter\gdef\csname claimval@infra.judge_incomplete\endcsname{69}
\expandafter\gdef\csname claimval@infra.zero_cost\endcsname{73}
\expandafter\gdef\csname claimval@jcap.affected_pct\endcsname{45}
\expandafter\gdef\csname claimval@jcap.completeness_floor\endcsname{0.80}
\expandafter\gdef\csname claimval@jcap.reverified_n\endcsname{18}
\expandafter\gdef\csname claimval@jn.band_mean\endcsname{0.0407}
\expandafter\gdef\csname claimval@jn.band_median\endcsname{0.0297}
\expandafter\gdef\csname claimval@jn.runs_with_split\endcsname{2{,}302}
\expandafter\gdef\csname claimval@jn.split_rate_pct\endcsname{8.5}
\expandafter\gdef\csname claimval@po.accept_rate_pct\endcsname{27.3}
\expandafter\gdef\csname claimval@po.exhausted_pct\endcsname{70.6}
\expandafter\gdef\csname claimval@po.max_round_share_pct\endcsname{82.4}
\expandafter\gdef\csname claimval@po.n_items\endcsname{344}
\expandafter\gdef\csname claimval@po.rounds_parsed\endcsname{239}
\expandafter\gdef\csname claimval@po.trough_share_pct\endcsname{5.8}
\expandafter\gdef\csname claimval@q0.crossing_far_pct\endcsname{0.0}
\expandafter\gdef\csname claimval@q0.crossing_near_n\endcsname{88}
\expandafter\gdef\csname claimval@q0.crossing_near_pct\endcsname{88.6}
\expandafter\gdef\csname claimval@q0.crossing_pct\endcsname{28.8}
\expandafter\gdef\csname claimval@q0.exact_match_pct\endcsname{5.0}
\expandafter\gdef\csname claimval@q0.n_groups\endcsname{685}
\expandafter\gdef\csname claimval@q0.n_groups_2\endcsname{66}
\expandafter\gdef\csname claimval@q0.n_groups_3\endcsname{619}
\expandafter\gdef\csname claimval@q0.n_measurements\endcsname{1,989}
\expandafter\gdef\csname claimval@q0.sigma_median\endcsname{0.085}
\expandafter\gdef\csname claimval@q0.sm_crossing_pct\endcsname{23.9}
\expandafter\gdef\csname claimval@q0.sm_excluded_crossing_pct\endcsname{32.6}
\expandafter\gdef\csname claimval@q0.sm_excluded_n\endcsname{380}
\expandafter\gdef\csname claimval@q0.sm_excluded_pct\endcsname{55.5}
\expandafter\gdef\csname claimval@q0.sm_excluded_verdict_pct\endcsname{0.1}
\expandafter\gdef\csname claimval@q0.sm_far_pct\endcsname{0.0}
\expandafter\gdef\csname claimval@q0.sm_n_groups\endcsname{305}
\expandafter\gdef\csname claimval@q0.sm_n_measurements\endcsname{876}
\expandafter\gdef\csname claimval@q0.sm_near_n\endcsname{45}
\expandafter\gdef\csname claimval@q0.sm_near_pct\endcsname{80.0}
\expandafter\gdef\csname claimval@q0.sm_sigma_median\endcsname{0.065}
\expandafter\gdef\csname claimval@q0.sm_exact_match_pct\endcsname{8.9}
\expandafter\gdef\csname claimval@q0.sm_spread_median\endcsname{0.148}
\expandafter\gdef\csname claimval@q0.spread_gt10_pct\endcsname{75.9}
\expandafter\gdef\csname claimval@q0.spread_gt20_pct\endcsname{47.9}
\expandafter\gdef\csname claimval@q0.spread_max\endcsname{1.000}
\expandafter\gdef\csname claimval@q0.spread_mean\endcsname{0.233}
\expandafter\gdef\csname claimval@q0.spread_median\endcsname{0.192}
\expandafter\gdef\csname claimval@q0.spread_median_2\endcsname{0.141}
\expandafter\gdef\csname claimval@q0.spread_median_3\endcsname{0.196}
\expandafter\gdef\csname claimval@q0.spread_p75\endcsname{0.319}
\expandafter\gdef\csname claimval@q0.spread_p90\endcsname{0.472}
\expandafter\gdef\csname claimval@q0.z_flagged\endcsname{68}
\expandafter\gdef\csname claimval@q0.z_paid\endcsname{292}
\expandafter\gdef\csname claimval@q0.z_suspect\endcsname{5}
\expandafter\gdef\csname claimval@q0.z_total\endcsname{365}
\expandafter\gdef\csname claimval@q1.bridge_factor\endcsname{4/9}
\expandafter\gdef\csname claimval@q1.crossing_ci_hi\endcsname{49.5}
\expandafter\gdef\csname claimval@q1.crossing_ci_lo\endcsname{10.2}
\expandafter\gdef\csname claimval@q1.crossing_k1_pct\endcsname{11.2}
\expandafter\gdef\csname claimval@q1.crossing_k5_pct\endcsname{8.3}
\expandafter\gdef\csname claimval@q1.paired_k_drop_pp\endcsname{2.87}
\expandafter\gdef\csname claimval@q1.paired_k_drop_lo\endcsname{0.73}
\expandafter\gdef\csname claimval@q1.paired_k_drop_hi\endcsname{5.51}
\expandafter\gdef\csname claimval@q1.paired_k_n_moved\endcsname{4}
\expandafter\gdef\csname claimval@q1.analytic_k_drop_per_group_pp\endcsname{11.28}
\expandafter\gdef\csname claimval@q1.analytic_k_drop_pp\endcsname{2.82}
\expandafter\gdef\csname claimval@q1.crossing_nozero_pct\endcsname{16.7}
\expandafter\gdef\csname claimval@q1.crossing_pct\endcsname{25.0}
\expandafter\gdef\csname claimval@q1.exemplar_n\endcsname{3}
\expandafter\gdef\csname claimval@q1.exemplar_scores\endcsname{0.139, 0.557, 0.639}
\expandafter\gdef\csname claimval@q1.min_k_for_5pct\endcsname{none}
\expandafter\gdef\csname claimval@q1.n_groups\endcsname{16}
\expandafter\gdef\csname claimval@q1.n_groups_nozero\endcsname{12}
\expandafter\gdef\csname claimval@q1.n_measurements\endcsname{52}
\expandafter\gdef\csname claimval@q1.naive_gap\endcsname{-0.20}
\expandafter\gdef\csname claimval@q1.sigma_median\endcsname{0.093}
\expandafter\gdef\csname claimval@q1.spread_median\endcsname{0.227}
\expandafter\gdef\csname claimval@q2.n_items\endcsname{47}
\expandafter\gdef\csname claimval@rep.max\endcsname{0.5772}
\expandafter\gdef\csname claimval@rep.median\endcsname{0.0556}
\expandafter\gdef\csname claimval@rep.median_ex_infra\endcsname{0.0509}
\expandafter\gdef\csname claimval@rep.n_copied\endcsname{3}
\expandafter\gdef\csname claimval@rep.n_ex_infra\endcsname{10}
\expandafter\gdef\csname claimval@rep.n_pairs\endcsname{12}
\expandafter\gdef\csname claimval@run.n\endcsname{3{,}862}
\expandafter\gdef\csname claimval@seed.n_models\endcsname{21}
\expandafter\gdef\csname claimval@tau.crossing_ge20_hi\endcsname{0.88}
\expandafter\gdef\csname claimval@tau.crossing_floor_pct\endcsname{20}
\expandafter\gdef\csname claimval@tau.crossing_ge20_lo\endcsname{0.16}
\expandafter\gdef\csname claimval@tau.crossing_peak_at\endcsname{0.68}
\expandafter\gdef\csname claimval@tau.crossing_peak_pct\endcsname{32.0}
\expandafter\gdef\csname claimval@xcheck.n_pairs\endcsname{8}
\expandafter\gdef\csname claimval@xcheck.agree_pct\endcsname{100.0}
\expandafter\gdef\csname claimval@xcheck.n_measurements\endcsname{20}
\expandafter\gdef\csname claimval@xcheck.n_items\endcsname{2}
\expandafter\gdef\csname claimval@q0.sm_n_crossing\endcsname{73}
\expandafter\gdef\csname claimval@gate.tau\endcsname{0.55}
\expandafter\gdef\csname claimval@xcheck.n_groups\endcsname{4}
\expandafter\gdef\csname claimval@xcheck.cross_pairs\endcsname{32}
\expandafter\gdef\csname claimval@xcheck.cross_missed\endcsname{12}
\expandafter\gdef\csname claimval@po.n_accepted\endcsname{94}
\expandafter\gdef\csname claimval@po.n_salvaged\endcsname{243}
\expandafter\gdef\csname claimval@pre.n_items\endcsname{100}
\expandafter\gdef\csname claimval@pre.n_domains\endcsname{11}
\expandafter\gdef\csname claimval@pre.n_scratch\endcsname{39}
\expandafter\gdef\csname claimval@pre.n_regen\endcsname{37}
\expandafter\gdef\csname claimval@pre.n_convert\endcsname{24}
\expandafter\gdef\csname claimval@case.saved_window_min\endcsname{739}
\expandafter\gdef\csname claimval@case.emitted_window_min\endcsname{737}
\expandafter\gdef\csname claimval@prospective.n_families\endcsname{67}
\expandafter\gdef\csname claimval@prospective.n_policies\endcsname{3}
\expandafter\gdef\csname claimval@prospective.n_cells\endcsname{201}
\expandafter\gdef\csname claimval@prospective.opportunities_per_cell\endcsname{2}
\expandafter\gdef\csname claimval@prospective.max_selected_per_cell\endcsname{1}
\expandafter\gdef\csname claimval@prospective.ablation_max\endcsname{24}
\expandafter\gdef\csname claimval@prospective.ablation_conditions\endcsname{4}
\expandafter\gdef\csname claimval@prospective.repairs_per_condition\endcsname{1}
\expandafter\gdef\csname claimval@prospective.fresh_repeats\endcsname{2}
\expandafter\gdef\csname claimval@prospective.independent_reviewers\endcsname{2}
\expandafter\gdef\csname claimval@prospective.review_checks\endcsname{6}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T0.fail\endcsname{14}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T0.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T0.runs\endcsname{16}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T0.unknown\endcsname{2}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T0.warn\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T1.fail\endcsname{14}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T1.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T1.runs\endcsname{16}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T1.unknown\endcsname{1}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D0T1.warn\endcsname{1}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T0.fail\endcsname{14}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T0.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T0.runs\endcsname{16}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T0.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T0.warn\endcsname{2}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T1.fail\endcsname{14}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T1.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T1.runs\endcsname{16}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T1.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.D1T1.warn\endcsname{2}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.conditions\endcsname{4}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.d.cp_hi\endcsname{0.439115}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.d.cp_lo\endcsname{-0.454224}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.d.id_hi\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.d.id_lo\endcsname{-0.09375}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.fail\endcsname{56}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.fee_missing\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.h.cp_hi\endcsname{0.908240}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.h.cp_lo\endcsname{-0.900862}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.h.id_hi\endcsname{0.125}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.h.id_lo\endcsname{-0.0625}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.ledger_events\endcsname{127}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.ledgers\endcsname{64}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.packages\endcsname{16}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.policy_zero\endcsname{61}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.runs\endcsname{64}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.t.cp_hi\endcsname{0.450431}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.t.cp_lo\endcsname{-0.454120}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.t.id_hi\endcsname{0.03125}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.t.id_lo\endcsname{-0.0625}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.unknown\endcsname{3}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.usd\endcsname{1{,}180.0039}
\expandafter\gdef\csname claimval@prospective.a64_original_20260912.warn\endcsname{5}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.D.cells\endcsname{67}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.D.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.D.policy_zero\endcsname{47}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.D.primary_unknown\endcsname{20}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.D.selected_pending\endcsname{3}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.D.selection_unresolved\endcsname{17}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.G.cells\endcsname{67}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.G.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.G.policy_zero\endcsname{55}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.G.primary_unknown\endcsname{12}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.G.selected_pending\endcsname{7}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.G.selection_unresolved\endcsname{5}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.I.cells\endcsname{67}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.I.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.I.policy_zero\endcsname{50}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.I.primary_unknown\endcsname{17}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.I.selected_pending\endcsname{6}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.I.selection_unresolved\endcsname{11}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.cells\endcsname{201}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.dg.cp_hi\endcsname{0.455766}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.dg.cp_lo\endcsname{-0.323570}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.dg.id_hi\endcsname{0.298507}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.dg.id_lo\endcsname{-0.179104}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.di.cp_hi\endcsname{0.455766}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.di.cp_lo\endcsname{-0.407677}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.di.id_hi\endcsname{0.298507}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.di.id_lo\endcsname{-0.253731}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.families\endcsname{67}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.holm_hi\endcsname{1}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.holm_lo\endcsname{2^{-18}}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.policies\endcsname{3}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.policy_zero\endcsname{152}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.primary_unknown\endcsname{49}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.selected_pending\endcsname{16}
\expandafter\gdef\csname claimval@prospective.main201_original_20260912.selection_unresolved\endcsname{33}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.baseline.fail\endcsname{56}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.baseline.unknown\endcsname{3}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.baseline.warn\endcsname{5}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.changed_cells\endcsname{1}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.fail\endcsname{57}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.human_labels\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.policy_zero\endcsname{62}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.unknown\endcsname{2}
\expandafter\gdef\csname claimval@prospective.a64_tail_appended_20260912.warn\endcsname{5}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.tasks\endcsname{18}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.families\endcsname{11}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.planned\endcsname{108}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.completed\endcsname{42}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.scored\endcsname{29}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.unknown\endcsname{79}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.known_successes\endcsname{0}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Sol.planned\endcsname{36}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Sol.completed\endcsname{12}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Sol.scored\endcsname{8}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Sol.identity_attributed\endcsname{35}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Sol.weighted_score.mean_bounds.lo\endcsname{0.158258}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Sol.weighted_score.mean_bounds.hi\endcsname{0.938561}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Luna.planned\endcsname{36}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Luna.completed\endcsname{20}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Luna.scored\endcsname{13}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Luna.identity_attributed\endcsname{36}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Luna.weighted_score.mean_bounds.lo\endcsname{0.161621}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Luna.weighted_score.mean_bounds.hi\endcsname{0.873742}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Gemini.planned\endcsname{36}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Gemini.completed\endcsname{10}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Gemini.scored\endcsname{8}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Gemini.identity_attributed\endcsname{18}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Gemini.weighted_score.mean_bounds.lo\endcsname{0.102856}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.Gemini.weighted_score.mean_bounds.hi\endcsname{0.883159}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.success.Sol_Luna.identification_bounds.lo\endcsname{-0.712121}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.success.Sol_Luna.identification_bounds.hi\endcsname{0.780303}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.success.Sol_Gemini.identification_bounds.lo\endcsname{-0.780303}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.success.Sol_Gemini.identification_bounds.hi\endcsname{0.780303}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.success.Luna_Gemini.identification_bounds.lo\endcsname{-0.780303}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.success.Luna_Gemini.identification_bounds.hi\endcsname{0.712121}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.weighted_score.Sol_Luna.identification_bounds.lo\endcsname{-0.715485}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.weighted_score.Sol_Luna.identification_bounds.hi\endcsname{0.776939}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.weighted_score.Sol_Gemini.identification_bounds.lo\endcsname{-0.724902}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.weighted_score.Sol_Gemini.identification_bounds.hi\endcsname{0.835705}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.weighted_score.Luna_Gemini.identification_bounds.lo\endcsname{-0.721538}
\expandafter\gdef\csname claimval@prospective.hu_20260912.U.weighted_score.Luna_Gemini.identification_bounds.hi\endcsname{0.770886}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.tasks\endcsname{16}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.families\endcsname{11}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.planned\endcsname{96}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.completed\endcsname{32}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.scored\endcsname{25}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.unknown\endcsname{71}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Sol.planned\endcsname{32}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Sol.completed\endcsname{8}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Sol.scored\endcsname{6}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Sol.identity_attributed\endcsname{31}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Sol.weighted_score.mean_bounds.lo\endcsname{0.152705}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Sol.weighted_score.mean_bounds.hi\endcsname{0.948159}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Luna.planned\endcsname{32}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Luna.completed\endcsname{16}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Luna.scored\endcsname{11}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Luna.identity_attributed\endcsname{32}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Luna.weighted_score.mean_bounds.lo\endcsname{0.169023}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Luna.weighted_score.mean_bounds.hi\endcsname{0.873568}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Gemini.planned\endcsname{32}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Gemini.completed\endcsname{8}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Gemini.scored\endcsname{8}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Gemini.identity_attributed\endcsname{14}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Gemini.weighted_score.mean_bounds.lo\endcsname{0.122114}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.Gemini.weighted_score.mean_bounds.hi\endcsname{0.872114}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.success.Sol_Luna.identification_bounds.lo\endcsname{-0.704545}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.success.Sol_Luna.identification_bounds.hi\endcsname{0.795455}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.success.Sol_Gemini.identification_bounds.lo\endcsname{-0.750000}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.success.Sol_Gemini.identification_bounds.hi\endcsname{0.795455}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.success.Luna_Gemini.identification_bounds.lo\endcsname{-0.750000}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.success.Luna_Gemini.identification_bounds.hi\endcsname{0.704545}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.weighted_score.Sol_Luna.identification_bounds.lo\endcsname{-0.720864}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.weighted_score.Sol_Luna.identification_bounds.hi\endcsname{0.779136}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.weighted_score.Sol_Gemini.identification_bounds.lo\endcsname{-0.719409}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.weighted_score.Sol_Gemini.identification_bounds.hi\endcsname{0.826045}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.weighted_score.Luna_Gemini.identification_bounds.lo\endcsname{-0.703091}
\expandafter\gdef\csname claimval@prospective.hu_20260912.R.weighted_score.Luna_Gemini.identification_bounds.hi\endcsname{0.751455}
\expandafter\gdef\csname claimval@prospective.hu_20260912.interval_envelope.lo\endcsname{-1.000000}
\expandafter\gdef\csname claimval@prospective.hu_20260912.interval_envelope.hi\endcsname{1.000000}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.synthetic_tasks\endcsname{2}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.planned_outputs\endcsname{5}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.planned_caps\endcsname{8}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.votes_per_cap\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.planned_ballots\endcsname{24}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.attempted_outputs\endcsname{5}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.complete_outputs\endcsname{4}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.partial_outputs\endcsname{1}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.html_browse_failures\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_001.J7.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_001.J7.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_001.J7.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_001.J8.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_001.J8.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_001.J8.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_002.J10.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_002.J10.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_002.J10.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_003.J7.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_003.J7.fail\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_003.J7.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_003.J8.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_003.J8.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_003.J8.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_004.J7.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_004.J7.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_004.J7.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_004.J8.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_004.J8.fail\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_004.J8.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_005.J10.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_005.J10.fail\endcsname{2}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.case_005.J10.unknown\endcsname{1}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.pass_ballots\endcsname{15}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.fail_ballots\endcsname{8}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.unknown_ballots\endcsname{1}
\expandafter\gdef\csname claimval@prospective.judge_controls_v1_20260912.valid_ballots\endcsname{23}
\expandafter\gdef\csname claimval@hja.all_n\endcsname{2,942}
\expandafter\gdef\csname claimval@hja.all_agree\endcsname{2,867}
\expandafter\gdef\csname claimval@hja.all_pct\endcsname{97.45}
\expandafter\gdef\csname claimval@hja.daily_n\endcsname{2,939}
\expandafter\gdef\csname claimval@hja.daily_agree\endcsname{2,864}
\expandafter\gdef\csname claimval@hja.daily_disagree\endcsname{75}
\expandafter\gdef\csname claimval@hja.daily_pct\endcsname{97.45}
\expandafter\gdef\csname claimval@hja.binary_n\endcsname{2,837}
\expandafter\gdef\csname claimval@hja.binary_agree\endcsname{2,762}
\expandafter\gdef\csname claimval@hja.binary_disagree\endcsname{75}
\expandafter\gdef\csname claimval@hja.binary_pct\endcsname{97.36}
\expandafter\gdef\csname claimval@hja.n_items\endcsname{150}
\expandafter\gdef\csname claimval@hja.n_tasks\endcsname{152}
\expandafter\gdef\csname claimval@hja.n_item_model_task_groups\endcsname{210}
\expandafter\gdef\csname claimval@hja.n_reviewers\endcsname{5}
\expandafter\gdef\csname claimval@hja.n_solver_labels\endcsname{4}
\expandafter\gdef\csname claimval@hja.pass_n\endcsname{1,154}
\expandafter\gdef\csname claimval@hja.pass_agree\endcsname{1,108}
\expandafter\gdef\csname claimval@hja.pass_disagree\endcsname{46}
\expandafter\gdef\csname claimval@hja.pass_pct\endcsname{96.01}
\expandafter\gdef\csname claimval@hja.fail_n\endcsname{1,683}
\expandafter\gdef\csname claimval@hja.fail_agree\endcsname{1,654}
\expandafter\gdef\csname claimval@hja.fail_disagree\endcsname{29}
\expandafter\gdef\csname claimval@hja.fail_pct\endcsname{98.28}
\expandafter\gdef\csname claimval@hja.excluded_n\endcsname{102}
\expandafter\gdef\csname claimval@hja.excluded_agree\endcsname{102}
\expandafter\gdef\csname claimval@hja.excluded_disagree\endcsname{0}
\expandafter\gdef\csname claimval@hja.excluded_pct\endcsname{100.00}
\expandafter\gdef\csname claimval@hja.item_macro_pct\endcsname{97.49}
\expandafter\gdef\csname claimval@hja.reviewer_macro_pct\endcsname{97.51}
\expandafter\gdef\csname claimval@hja.reviewer_rate_min_pct\endcsname{96.33}
\expandafter\gdef\csname claimval@hja.reviewer_rate_max_pct\endcsname{98.16}
\expandafter\gdef\csname claimval@hja.ci_lo_pct\endcsname{96.42}
\expandafter\gdef\csname claimval@hja.ci_hi_pct\endcsname{98.26}
\expandafter\gdef\csname claimval@hja.bootstrap_n\endcsname{20,000}
\expandafter\gdef\csname claimval@hja.bootstrap_seed\endcsname{20260917}
\expandafter\gdef\csname claimval@hja.ci_level\endcsname{95}
\expandafter\gdef\csname claimval@hja2.all_n\endcsname{8,338}
\expandafter\gdef\csname claimval@hja2.binary_agree\endcsname{7,429}
\expandafter\gdef\csname claimval@hja2.binary_disagree\endcsname{274}
\expandafter\gdef\csname claimval@hja2.binary_n\endcsname{7,703}
\expandafter\gdef\csname claimval@hja2.binary_pct\endcsname{96.44}
\expandafter\gdef\csname claimval@hja2.bootstrap_n\endcsname{20,000}
\expandafter\gdef\csname claimval@hja2.bootstrap_seed\endcsname{20260920}
\expandafter\gdef\csname claimval@hja2.ci_hi_pct\endcsname{97.03}
\expandafter\gdef\csname claimval@hja2.ci_level\endcsname{95}
\expandafter\gdef\csname claimval@hja2.ci_lo_pct\endcsname{95.88}
\expandafter\gdef\csname claimval@hja2.daily_agree\endcsname{7,539}
\expandafter\gdef\csname claimval@hja2.daily_disagree\endcsname{276}
\expandafter\gdef\csname claimval@hja2.daily_n\endcsname{7,815}
\expandafter\gdef\csname claimval@hja2.daily_pct\endcsname{96.47}
\expandafter\gdef\csname claimval@hja2.excluded_agree\endcsname{102}
\expandafter\gdef\csname claimval@hja2.excluded_disagree\endcsname{0}
\expandafter\gdef\csname claimval@hja2.excluded_n\endcsname{102}
\expandafter\gdef\csname claimval@hja2.excluded_pct\endcsname{100.00}
\expandafter\gdef\csname claimval@hja2.fail_agree\endcsname{4,629}
\expandafter\gdef\csname claimval@hja2.fail_disagree\endcsname{57}
\expandafter\gdef\csname claimval@hja2.fail_n\endcsname{4,686}
\expandafter\gdef\csname claimval@hja2.fail_pct\endcsname{98.78}
\expandafter\gdef\csname claimval@hja2.item_macro_pct\endcsname{96.95}
\expandafter\gdef\csname claimval@hja2.missing_agree\endcsname{8}
\expandafter\gdef\csname claimval@hja2.missing_disagree\endcsname{2}
\expandafter\gdef\csname claimval@hja2.missing_n\endcsname{10}
\expandafter\gdef\csname claimval@hja2.missing_pct\endcsname{80.00}
\expandafter\gdef\csname claimval@hja2.n_items\endcsname{216}
\expandafter\gdef\csname claimval@hja2.n_reviewers\endcsname{9}
\expandafter\gdef\csname claimval@hja2.n_solver_labels\endcsname{10}
\expandafter\gdef\csname claimval@hja2.n_tasks\endcsname{300}
\expandafter\gdef\csname claimval@hja2.old_groups_agree\endcsname{2,904}
\expandafter\gdef\csname claimval@hja2.old_groups_n\endcsname{2,981}
\expandafter\gdef\csname claimval@hja2.old_groups_pct\endcsname{97.42}
\expandafter\gdef\csname claimval@hja2.pass_agree\endcsname{2,800}
\expandafter\gdef\csname claimval@hja2.pass_disagree\endcsname{217}
\expandafter\gdef\csname claimval@hja2.pass_n\endcsname{3,017}
\expandafter\gdef\csname claimval@hja2.pass_pct\endcsname{92.81}
\expandafter\gdef\csname claimval@hja2.qa_approved_agree\endcsname{6,501}
\expandafter\gdef\csname claimval@hja2.qa_approved_n\endcsname{6,758}
\expandafter\gdef\csname claimval@hja2.qa_approved_pct\endcsname{96.20}
\expandafter\gdef\csname claimval@hja2.qa_rejected_agree\endcsname{1}
\expandafter\gdef\csname claimval@hja2.qa_rejected_n\endcsname{2}
\expandafter\gdef\csname claimval@hja2.qa_rejected_pct\endcsname{50.00}
\expandafter\gdef\csname claimval@hja2.qa_unreviewed_agree\endcsname{1,037}
\expandafter\gdef\csname claimval@hja2.qa_unreviewed_n\endcsname{1,055}
\expandafter\gdef\csname claimval@hja2.qa_unreviewed_pct\endcsname{98.29}
\expandafter\gdef\csname claimval@hja2.reviewer_macro_pct\endcsname{96.53}
\expandafter\gdef\csname claimval@repair_case.n_packages\endcsname{1}
\expandafter\gdef\csname claimval@repair_case.n_conditions\endcsname{4}
\expandafter\gdef\csname claimval@repair_case.ballots_per_condition\endcsname{1}
\expandafter\gdef\csname claimval@repair_case.original_minutes\endcsname{320}
\expandafter\gdef\csname claimval@repair_case.corrected_minutes\endcsname{380}
\expandafter\gdef\csname claimval@release20.formats.PASS\endcsname{117}
\expandafter\gdef\csname claimval@release20.formats.supported_locations\endcsname{118}
\expandafter\gdef\csname claimval@release20.formats.unsupported_locations\endcsname{1025}
\expandafter\gdef\csname claimval@release20.operations.fetch.PASS\endcsname{76}
\expandafter\gdef\csname claimval@release20.operations.fetch.total\endcsname{77}
\expandafter\gdef\csname claimval@release20.operations.search.total\endcsname{106}
\expandafter\gdef\csname claimval@release20.package_checks.deterministic_evidence_binding.FAIL\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.deterministic_evidence_binding.PASS\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.deterministic_evidence_binding.UNKNOWN\endcsname{20}
\expandafter\gdef\csname claimval@release20.package_checks.deterministic_rubric_answer_consistency.FAIL\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.deterministic_rubric_answer_consistency.PASS\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.deterministic_rubric_answer_consistency.UNKNOWN\endcsname{20}
\expandafter\gdef\csname claimval@release20.package_checks.instruction_structure.FAIL\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.instruction_structure.PASS\endcsname{20}
\expandafter\gdef\csname claimval@release20.package_checks.instruction_structure.UNKNOWN\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.mapping_authentication.FAIL\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.mapping_authentication.PASS\endcsname{20}
\expandafter\gdef\csname claimval@release20.package_checks.mapping_authentication.UNKNOWN\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.production_local_mcp_fetch.FAIL\endcsname{1}
\expandafter\gdef\csname claimval@release20.package_checks.production_local_mcp_fetch.PASS\endcsname{16}
\expandafter\gdef\csname claimval@release20.package_checks.production_local_mcp_fetch.UNKNOWN\endcsname{3}
\expandafter\gdef\csname claimval@release20.package_checks.production_local_mcp_search.FAIL\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.production_local_mcp_search.PASS\endcsname{17}
\expandafter\gdef\csname claimval@release20.package_checks.production_local_mcp_search.UNKNOWN\endcsname{3}
\expandafter\gdef\csname claimval@release20.package_checks.public_workspace_reachability.FAIL\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.public_workspace_reachability.PASS\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.public_workspace_reachability.UNKNOWN\endcsname{20}
\expandafter\gdef\csname claimval@release20.package_checks.safe_file_openability.FAIL\endcsname{1}
\expandafter\gdef\csname claimval@release20.package_checks.safe_file_openability.PASS\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.safe_file_openability.UNKNOWN\endcsname{19}
\expandafter\gdef\csname claimval@release20.package_checks.semantic_correctness.FAIL\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.semantic_correctness.PASS\endcsname{0}
\expandafter\gdef\csname claimval@release20.package_checks.semantic_correctness.UNKNOWN\endcsname{20}
\expandafter\gdef\csname claimval@release20.population\endcsname{100}
\expandafter\gdef\csname claimval@release20.sampled\endcsname{20}
\expandafter\gdef\csname claimval@release20.unsampled\endcsname{80}
\expandafter\gdef\csname claimval@adj.N01\endcsname{19}
\expandafter\gdef\csname claimval@adj.N02\endcsname{14}
\expandafter\gdef\csname claimval@adj.N03\endcsname{564}
\expandafter\gdef\csname claimval@adj.N24\endcsname{two}
\expandafter\gdef\csname claimval@adj.N04\endcsname{17}
\expandafter\gdef\csname claimval@adj.N05\endcsname{seven}
\expandafter\gdef\csname claimval@adj.N06\endcsname{12}
\expandafter\gdef\csname claimval@adj.N07\endcsname{five}
\expandafter\gdef\csname claimval@adj.N08\endcsname{two}
\expandafter\gdef\csname claimval@adj.N09\endcsname{19}
\expandafter\gdef\csname claimval@adj.N10\endcsname{14}
\expandafter\gdef\csname claimval@adj.N11\endcsname{33}
\expandafter\gdef\csname claimval@adj.N12\endcsname{66}
\expandafter\gdef\csname claimval@adj.T18.snapshot_smax_pre\endcsname{0.395}
\expandafter\gdef\csname claimval@adj.T18.snapshot_smax_post\endcsname{0.622}
\expandafter\gdef\csname claimval@adj.N13\endcsname{8}
\expandafter\gdef\csname claimval@adj.N14\endcsname{6}
\expandafter\gdef\csname claimval@adj.N15\endcsname{6}
\expandafter\gdef\csname claimval@adj.N16\endcsname{38}
\expandafter\gdef\csname claimval@adj.N17\endcsname{21}
\expandafter\gdef\csname claimval@adj.N18\endcsname{13}
\expandafter\gdef\csname claimval@adj.N19\endcsname{4}
\expandafter\gdef\csname claimval@adj.N20\endcsname{27}
\expandafter\gdef\csname claimval@adj.N21\endcsname{2}
\expandafter\gdef\csname claimval@adj.N22\endcsname{17}
\expandafter\gdef\csname claimval@adj.N25\endcsname{0}
\expandafter\gdef\csname claimval@adj.T08.snapshot_wmax_pre\endcsname{0.672}
\expandafter\gdef\csname claimval@adj.T08.model_1_pre_score\endcsname{0.648}
\expandafter\gdef\csname claimval@adj.T04.pre_spec_criteria\endcsname{15}
\expandafter\gdef\csname claimval@adj.N23\endcsname{14}
\expandafter\gdef\csname claimval@adj.T04.pre_spec_weight\endcsname{129}
\expandafter\gdef\csname claimval@adj.T04.post_spec_weight\endcsname{138}
\expandafter\gdef\csname claimval@adj.T04.model_1_pre_scored_weight\endcsname{119}
\expandafter\gdef\csname claimval@adj.T04.model_1_post_scored_weight\endcsname{128}
\expandafter\gdef\csname claimval@adj.T01.snapshot_smax_pre\endcsname{0.462}
\expandafter\gdef\csname claimval@adj.T01.snapshot_smax_post\endcsname{0.579}
\expandafter\gdef\csname claimval@adj.T01.snapshot_wmax_pre\endcsname{0.276}
\expandafter\gdef\csname claimval@adj.T01.snapshot_wmax_post\endcsname{0.393}
\expandafter\gdef\csname claimval@adj.T01.pre_spec_weight\endcsname{145}
\expandafter\gdef\csname claimval@adj.T01.post_spec_weight\endcsname{145}
\expandafter\gdef\csname claimval@adj.T01.exact_retained_body_weight_count\endcsname{15}
\expandafter\gdef\csname claimval@adj.T02.snapshot_smax_pre\endcsname{0.789}
\expandafter\gdef\csname claimval@adj.T02.snapshot_smax_post\endcsname{0.441}
\expandafter\gdef\csname claimval@adj.T02.snapshot_wmax_pre\endcsname{0.555}
\expandafter\gdef\csname claimval@adj.T02.snapshot_wmax_post\endcsname{0.303}
\expandafter\gdef\csname claimval@adj.T02.pre_spec_weight\endcsname{128}
\expandafter\gdef\csname claimval@adj.T02.post_spec_weight\endcsname{145}
\expandafter\gdef\csname claimval@adj.T02.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T03.snapshot_smax_pre\endcsname{0.726}
\expandafter\gdef\csname claimval@adj.T03.snapshot_smax_post\endcsname{0.504}
\expandafter\gdef\csname claimval@adj.T03.snapshot_wmax_pre\endcsname{0.548}
\expandafter\gdef\csname claimval@adj.T03.snapshot_wmax_post\endcsname{0.304}
\expandafter\gdef\csname claimval@adj.T03.pre_spec_weight\endcsname{135}
\expandafter\gdef\csname claimval@adj.T03.post_spec_weight\endcsname{135}
\expandafter\gdef\csname claimval@adj.T03.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T04.snapshot_smax_pre\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T04.snapshot_smax_post\endcsname{0.844}
\expandafter\gdef\csname claimval@adj.T04.snapshot_wmax_pre\endcsname{0.370}
\expandafter\gdef\csname claimval@adj.T04.snapshot_wmax_post\endcsname{0.188}
\expandafter\gdef\csname claimval@adj.T04.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T05.snapshot_smax_pre\endcsname{0.915}
\expandafter\gdef\csname claimval@adj.T05.snapshot_smax_post\endcsname{0.568}
\expandafter\gdef\csname claimval@adj.T05.snapshot_wmax_pre\endcsname{0.458}
\expandafter\gdef\csname claimval@adj.T05.snapshot_wmax_post\endcsname{0.229}
\expandafter\gdef\csname claimval@adj.T05.pre_spec_weight\endcsname{118}
\expandafter\gdef\csname claimval@adj.T05.post_spec_weight\endcsname{118}
\expandafter\gdef\csname claimval@adj.T05.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T06.snapshot_smax_pre\endcsname{0.926}
\expandafter\gdef\csname claimval@adj.T06.snapshot_smax_post\endcsname{0.829}
\expandafter\gdef\csname claimval@adj.T06.snapshot_wmax_pre\endcsname{0.748}
\expandafter\gdef\csname claimval@adj.T06.snapshot_wmax_post\endcsname{0.757}
\expandafter\gdef\csname claimval@adj.T06.pre_spec_weight\endcsname{135}
\expandafter\gdef\csname claimval@adj.T06.post_spec_weight\endcsname{140}
\expandafter\gdef\csname claimval@adj.T06.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T07.snapshot_smax_pre\endcsname{0.829}
\expandafter\gdef\csname claimval@adj.T07.snapshot_smax_post\endcsname{0.754}
\expandafter\gdef\csname claimval@adj.T07.snapshot_wmax_pre\endcsname{0.757}
\expandafter\gdef\csname claimval@adj.T07.snapshot_wmax_post\endcsname{0.754}
\expandafter\gdef\csname claimval@adj.T07.pre_spec_weight\endcsname{140}
\expandafter\gdef\csname claimval@adj.T07.post_spec_weight\endcsname{138}
\expandafter\gdef\csname claimval@adj.T07.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T08.snapshot_smax_pre\endcsname{0.648}
\expandafter\gdef\csname claimval@adj.T08.snapshot_smax_post\endcsname{0.808}
\expandafter\gdef\csname claimval@adj.T08.snapshot_wmax_post\endcsname{0.808}
\expandafter\gdef\csname claimval@adj.T08.pre_spec_weight\endcsname{125}
\expandafter\gdef\csname claimval@adj.T08.post_spec_weight\endcsname{125}
\expandafter\gdef\csname claimval@adj.T08.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T09.snapshot_smax_pre\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T09.snapshot_smax_post\endcsname{0.688}
\expandafter\gdef\csname claimval@adj.T09.snapshot_wmax_pre\endcsname{0.351}
\expandafter\gdef\csname claimval@adj.T09.snapshot_wmax_post\endcsname{0.495}
\expandafter\gdef\csname claimval@adj.T09.pre_spec_weight\endcsname{114}
\expandafter\gdef\csname claimval@adj.T09.post_spec_weight\endcsname{109}
\expandafter\gdef\csname claimval@adj.T09.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T10.snapshot_smax_pre\endcsname{0.810}
\expandafter\gdef\csname claimval@adj.T10.snapshot_smax_post\endcsname{0.855}
\expandafter\gdef\csname claimval@adj.T10.snapshot_wmax_pre\endcsname{0.782}
\expandafter\gdef\csname claimval@adj.T10.snapshot_wmax_post\endcsname{0.732}
\expandafter\gdef\csname claimval@adj.T10.pre_spec_weight\endcsname{142}
\expandafter\gdef\csname claimval@adj.T10.post_spec_weight\endcsname{138}
\expandafter\gdef\csname claimval@adj.T10.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T11.snapshot_smax_pre\endcsname{0.855}
\expandafter\gdef\csname claimval@adj.T11.snapshot_smax_post\endcsname{0.829}
\expandafter\gdef\csname claimval@adj.T11.snapshot_wmax_pre\endcsname{0.732}
\expandafter\gdef\csname claimval@adj.T11.snapshot_wmax_post\endcsname{0.810}
\expandafter\gdef\csname claimval@adj.T11.pre_spec_weight\endcsname{138}
\expandafter\gdef\csname claimval@adj.T11.post_spec_weight\endcsname{158}
\expandafter\gdef\csname claimval@adj.T11.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T12.snapshot_smax_pre\endcsname{0.948}
\expandafter\gdef\csname claimval@adj.T12.snapshot_smax_post\endcsname{0.843}
\expandafter\gdef\csname claimval@adj.T12.snapshot_wmax_pre\endcsname{0.674}
\expandafter\gdef\csname claimval@adj.T12.snapshot_wmax_post\endcsname{0.686}
\expandafter\gdef\csname claimval@adj.T12.pre_spec_weight\endcsname{135}
\expandafter\gdef\csname claimval@adj.T12.post_spec_weight\endcsname{172}
\expandafter\gdef\csname claimval@adj.T12.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T13.snapshot_smax_pre\endcsname{0.843}
\expandafter\gdef\csname claimval@adj.T13.snapshot_smax_post\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T13.snapshot_wmax_pre\endcsname{0.686}
\expandafter\gdef\csname claimval@adj.T13.snapshot_wmax_post\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T13.pre_spec_weight\endcsname{172}
\expandafter\gdef\csname claimval@adj.T13.post_spec_weight\endcsname{162}
\expandafter\gdef\csname claimval@adj.T13.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T14.snapshot_smax_pre\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T14.snapshot_smax_post\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T14.snapshot_wmax_pre\endcsname{0.897}
\expandafter\gdef\csname claimval@adj.T14.snapshot_wmax_post\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T14.pre_spec_weight\endcsname{165}
\expandafter\gdef\csname claimval@adj.T14.post_spec_weight\endcsname{162}
\expandafter\gdef\csname claimval@adj.T14.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T15.snapshot_smax_pre\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T15.snapshot_smax_post\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T15.snapshot_wmax_pre\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T15.snapshot_wmax_post\endcsname{1.000}
\expandafter\gdef\csname claimval@adj.T15.pre_spec_weight\endcsname{162}
\expandafter\gdef\csname claimval@adj.T15.post_spec_weight\endcsname{165}
\expandafter\gdef\csname claimval@adj.T15.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T16.snapshot_smax_pre\endcsname{0.789}
\expandafter\gdef\csname claimval@adj.T16.snapshot_smax_post\endcsname{0.784}
\expandafter\gdef\csname claimval@adj.T16.snapshot_wmax_pre\endcsname{0.680}
\expandafter\gdef\csname claimval@adj.T16.snapshot_wmax_post\endcsname{0.648}
\expandafter\gdef\csname claimval@adj.T16.pre_spec_weight\endcsname{128}
\expandafter\gdef\csname claimval@adj.T16.post_spec_weight\endcsname{125}
\expandafter\gdef\csname claimval@adj.T16.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T17.snapshot_smax_pre\endcsname{0.908}
\expandafter\gdef\csname claimval@adj.T17.snapshot_smax_post\endcsname{0.395}
\expandafter\gdef\csname claimval@adj.T17.snapshot_wmax_pre\endcsname{0.375}
\expandafter\gdef\csname claimval@adj.T17.snapshot_wmax_post\endcsname{0.105}
\expandafter\gdef\csname claimval@adj.T17.pre_spec_weight\endcsname{152}
\expandafter\gdef\csname claimval@adj.T17.post_spec_weight\endcsname{162}
\expandafter\gdef\csname claimval@adj.T17.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T18.snapshot_wmax_pre\endcsname{0.105}
\expandafter\gdef\csname claimval@adj.T18.snapshot_wmax_post\endcsname{0.052}
\expandafter\gdef\csname claimval@adj.T18.pre_spec_weight\endcsname{162}
\expandafter\gdef\csname claimval@adj.T18.post_spec_weight\endcsname{135}
\expandafter\gdef\csname claimval@adj.T18.exact_retained_body_weight_count\endcsname{0}
\expandafter\gdef\csname claimval@adj.T19.snapshot_smax_pre\endcsname{0.348}
\expandafter\gdef\csname claimval@adj.T19.snapshot_smax_post\endcsname{0.261}
\expandafter\gdef\csname claimval@adj.T19.snapshot_wmax_pre\endcsname{0.261}
\expandafter\gdef\csname claimval@adj.T19.snapshot_wmax_post\endcsname{0.261}
\expandafter\gdef\csname claimval@adj.T19.pre_spec_weight\endcsname{115}
\expandafter\gdef\csname claimval@adj.T19.post_spec_weight\endcsname{115}
\expandafter\gdef\csname claimval@adj.T19.exact_retained_body_weight_count\endcsname{12}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.planned_ballots\endcsname{24}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.valid_ballots\endcsname{21}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.pass_ballots\endcsname{15}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.fail_ballots\endcsname{6}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.unknown_ballots\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.criteria_total\endcsname{8}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.criteria_complete\endcsname{7}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.cases_total\endcsname{5}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.cases_complete\endcsname{4}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_001.J7.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_001.J7.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_001.J7.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_001.J8.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_001.J8.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_001.J8.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_002.J10.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_002.J10.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_002.J10.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_003.J7.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_003.J7.fail\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_003.J7.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_003.J8.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_003.J8.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_003.J8.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_004.J7.pass\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_004.J7.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_004.J7.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_004.J8.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_004.J8.fail\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_004.J8.unknown\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_005.J10.pass\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_005.J10.fail\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.case_005.J10.unknown\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.browse_walkthroughs\endcsname{6}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.browse_votes_per_html\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.functional_dom_changed\endcsname{3}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.noop_dom_changed\endcsname{0}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.http_requests\endcsname{133}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.http_text\endcsname{105}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.http_vision\endcsname{28}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.usage_unknown_requests\endcsname{1}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.known_total_tokens\endcsname{1947646}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.image_records\endcsname{43}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.per_ballot_http_max\endcsname{8}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.per_ballot_tool_max\endcsname{16}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.per_ballot_seconds\endcsname{180}
\expandafter\gdef\csname claimval@prospective.judge_controls_r310_20260928.immutable_consumed_slots\endcsname{19}
\makeatother


% Original full-cohort constants for inactive archive text only.
\expandafter\gdef\csname claimval@archive24.cap.alpha_pct\endcsname{5}
\expandafter\gdef\csname claimval@archive24.cap.bottom_overall\endcsname{40.4\%}
\expandafter\gdef\csname claimval@archive24.cap.cell_max\endcsname{92}
\expandafter\gdef\csname claimval@archive24.cap.cell_min\endcsname{10}
\expandafter\gdef\csname claimval@archive24.cap.hardest_fail_pct\endcsname{88.1}
\expandafter\gdef\csname claimval@archive24.cap.hardest_id\endcsname{Y11}
\expandafter\gdef\csname claimval@archive24.cap.hardest_n\endcsname{544}
\expandafter\gdef\csname claimval@archive24.cap.n_below_half_pool\endcsname{8}
\expandafter\gdef\csname claimval@archive24.cap.n_cells\endcsname{264}
\expandafter\gdef\csname claimval@archive24.cap.n_degenerate\endcsname{0}
\expandafter\gdef\csname claimval@archive24.cap.n_double_median\endcsname{18}
\expandafter\gdef\csname claimval@archive24.cap.n_eff_short\endcsname{6}
\expandafter\gdef\csname claimval@archive24.cap.n_floor\endcsname{6}
\expandafter\gdef\csname claimval@archive24.cap.n_graded\endcsname{55,143}
\expandafter\gdef\csname claimval@archive24.cap.n_imputed_cells\endcsname{3}
\expandafter\gdef\csname claimval@archive24.cap.n_items\endcsname{100}
\expandafter\gdef\csname claimval@archive24.cap.n_max_subset\endcsname{17}
\expandafter\gdef\csname claimval@archive24.cap.n_median_subset\endcsname{9}
\expandafter\gdef\csname claimval@archive24.cap.n_min_subset\endcsname{2}
\expandafter\gdef\csname claimval@archive24.cap.n_models\endcsname{24}
\expandafter\gdef\csname claimval@archive24.cap.n_models_ran_short\endcsname{1}
\expandafter\gdef\csname claimval@archive24.cap.n_models_sentinel\endcsname{2}
\expandafter\gdef\csname claimval@archive24.cap.n_models_short\endcsname{3}
\expandafter\gdef\csname claimval@archive24.cap.n_pairs\endcsname{276}
\expandafter\gdef\csname claimval@archive24.cap.n_rows\endcsname{56{,}153}
\expandafter\gdef\csname claimval@archive24.cap.n_starved\endcsname{1}
\expandafter\gdef\csname claimval@archive24.cap.n_subsets\endcsname{11}
\expandafter\gdef\csname claimval@archive24.cap.n_wider_span\endcsname{10}
\expandafter\gdef\csname claimval@archive24.cap.rho_median\endcsname{0.77}
\expandafter\gdef\csname claimval@archive24.cap.rho_min\endcsname{0.55}
\expandafter\gdef\csname claimval@archive24.cap.sep_double_median_pct\endcsname{45}
\expandafter\gdef\csname claimval@archive24.cap.sep_max_pct\endcsname{45}
\expandafter\gdef\csname claimval@archive24.cap.sep_median_pct\endcsname{31}
\expandafter\gdef\csname claimval@archive24.cap.sep_min_pct\endcsname{0}
\expandafter\gdef\csname claimval@archive24.cap.sep_pool_pct\endcsname{76}
\expandafter\gdef\csname claimval@archive24.cap.top_overall\endcsname{78.2\%}
\expandafter\gdef\csname claimval@archive24.seed.ci_width_max\endcsname{10}
\expandafter\gdef\csname claimval@archive24.seed.ci_width_min\endcsname{3}
\expandafter\gdef\csname claimval@archive24.seed.gap_median\endcsname{0.015}
\expandafter\gdef\csname claimval@archive24.seed.half_width\endcsname{0.073}
\expandafter\gdef\csname claimval@archive24.seed.half_width_paired\endcsname{0.055}
\expandafter\gdef\csname claimval@archive24.seed.imp_rank_from\endcsname{17}
\expandafter\gdef\csname claimval@archive24.seed.imp_rank_to\endcsname{15}
\expandafter\gdef\csname claimval@archive24.seed.mean_inversions\endcsname{6.8}
\expandafter\gdef\csname claimval@archive24.seed.n_adjacent\endcsname{23}
\expandafter\gdef\csname claimval@archive24.seed.n_basis_changed\endcsname{5}
\expandafter\gdef\csname claimval@archive24.seed.n_common_items\endcsname{92}
\expandafter\gdef\csname claimval@archive24.seed.n_inseparable\endcsname{23}
\expandafter\gdef\csname claimval@archive24.seed.n_items\endcsname{100}
\expandafter\gdef\csname claimval@archive24.seed.n_models\endcsname{24}
\expandafter\gdef\csname claimval@archive24.seed.n_pipeline_items\endcsname{369}
\expandafter\gdef\csname claimval@archive24.seed.n_single_shot_pairs\endcsname{264}
\expandafter\gdef\csname claimval@archive24.seed.n_tied_leader\endcsname{6}
\expandafter\gdef\csname claimval@archive24.seed.n_width_lt3\endcsname{0}
\expandafter\gdef\csname claimval@archive24.seed.p_preserved_pct\endcsname{0.00}
\expandafter\gdef\csname claimval@archive24.seed.p_top1_pct\endcsname{80.2}
\expandafter\gdef\csname claimval@archive24.seed.sd_median\endcsname{0.262}
\expandafter\gdef\csname claimval@archive24.seed.pair_common_min\endcsname{94}
\expandafter\gdef\csname claimval@archive24.seed.pair_common_max\endcsname{100}
\expandafter\gdef\csname claimval@archive24.seed.n_domains\endcsname{4}

